Neural Polar Decoders for DNA Data Storage

Synchronization errors, such as insertions and deletions, present a fundamental challenge in DNA-based data storage systems, arising from both synthesis and sequencing noise. These channels are often modeled as insertion-deletion-substitution (IDS) channels, for which designing maximum-likelihood decoders is computationally expensive. In this work, we propose a data-driven approach based on neural polar decoders (NPDs) to design low-complexity decoders for channels with synchronization errors. The proposed architecture enables decoding over IDS channels with reduced complexity $O(AN log N )$, where $A$ is a tunable parameter independent of the channel. NPDs require only sample access to the channel and can be trained without an explicit channel model. Additionally, NPDs provide mutual information (MI) estimates that can be used to optimize input distributions and code design. We demonstrate the effectiveness of NPDs on both synthetic deletion and IDS channels. For deletion channels, we show that NPDs achieve near-optimal decoding performance and accurate MI estimation, with significantly lower complexity than trellis-based decoders. We also provide numerical estimates of the channel capacity for the deletion channel. We extend our evaluation to realistic DNA storage settings, including channels with multiple noisy reads and real-world Nanopore sequencing data. Our results show that NPDs match or surpass the performance of existing methods while using significantly fewer parameters than the state-of-the-art. These findings highlight the promise of NPDs for robust and efficient decoding in DNA data storage systems.

==> figures/diagrams/communication-setting.tex <==
\begin{tikzpicture}[node distance=3.8cm and 2.5cm, auto, >=Latex]
    \node[minimum width=0.5cm, minimum height=1cm] (m) {$M$};
    \node[draw, rectangle, right=1.cm of m, minimum width=1.5cm, minimum height=1cm] (enc) {Encoder};
    \node[draw, rectangle, right=1.5cm of enc, minimum width=1.5cm, minimum height=1cm] (ch) {Channel};
    \node[draw, rectangle, below=0.5cm of ch, minimum width=0.5cm, minimum height=0.5cm] (del) {$\Delta$};
    \node[draw, rectangle, right=1.5cm of ch, minimum width=1.5cm, minimum height=1cm] (dec) {Decoder};
    \node[right=0.5cm of dec, minimum width=0.5cm, minimum height=1cm] (mhat) {$\hat{M}$};
  
    % Arrows
    \draw[->] (m.east) --  (enc.west);
    \draw[->] (enc.east) -- node[above] {$X^N$} (ch.west);
    \draw[->] (ch.east) -- node[above](y) {$Y^N$} (dec.west);
    \draw[->] (y.south) |- (del.east);
    \draw[->, dashed] (del.west) -| (enc.south);
    \draw[->] (ch.east) -- node[above] {} (dec.west);
    \draw[->] (dec.east) --  (mhat.west);
    % \draw[->, thick] (3,1) .. controls (2.5,0.5) and (1,-0.5) .. (0.2,-1);

    % \draw[->] (dec.east) to[bend right=30] node[below] {Feedback} (enc.south);
  \end{tikzpicture}

==> figures/diagrams/trellis-deletion.tex <==
\begin{tikzpicture}
    \foreach \x in {0.5, 2.5, 4.5, 6.5} {
        \fill[yellow!50] (\x, -3.5) rectangle ++(1, 7.5);
    }
    % Nodes for x values on the left
    \node[] at (1, 4.5) {$x_1$};
    \node[] at (3, 4.5) {$x_2$};
    \node[] at (5, 4.5) {$x_3$};
    \node[] at (7, 4.5) {$x_4$};
    % Nodes for y values on the left
    \node[blue] at (-1, 2) {$y_1 = 1$};
    \node[red] at (-1, 0) {$y_2 = 0$};
    \node[blue] at (-1, -2) {$y_3 = 1$};

    % Nodes representing dots
    \foreach \y in {3, 1, -1, -3} {
        \foreach \x in {0, 2, 4, 6, 8} {
            \node[circle, fill=black, inner sep=1pt] at (\x, \y) {};
        }
    }
    \draw (0, 3) circle (0.15cm);
    \draw (8, -3) circle (0.15cm);
    % Draw arrows with annotations
    % Red arrow from (0, 3) to (2, 1)
    \draw[->, red, thick] (0, 3) to[out=45, in=135]node[midway, above] {$\scriptstyled / 2$}(2, 3);
    \draw[->, blue, thick] (0, 3) to[out=-45, in=-135]node[midway, above] {$\scriptstyled / 2$}(2, 3);
    \draw[->, blue, thick] (0, 3) tonode[midway, above] {$\scriptstyle\bar{d} / 2$}(2, 1);
    \draw[->, blue, thick] (2, 3) tonode[midway, above] {$\scriptstyle\bar{d} / 2$}(4, 1);
    
    \draw[->, red, thick] (2, 1) to[out=45, in=135]node[midway, above] {$\scriptstyled / 2$}(4, 1);
    \draw[->, blue, thick] (2, 1) to[out=-45, in=-135]node[midway, above] {$\scriptstyled / 2$}(4, 1);
    \draw[->, red, thick] (2, 1) tonode[midway, above] {$\scriptstyle\bar{d} / 2$}(4, -1);
    \draw[->, red, thick] (4, 1) tonode[midway, above] {$\scriptstyle\bar{d} / 2$}(6, -1);


    \draw[->, red, thick] (4, -1) to[out=45, in=135]node[midway, above] {$\scriptstyled / 2$}(6, -1);
    \draw[->, blue, thick] (4, -1) to[out=-45, in=-135]node[midway, above] {$\scriptstyled / 2$}(6, -1);
    \draw[->, blue, thick] (4, -1) tonode[midway, above] {$\scriptstyle\bar{d} / 2$}(6, -3);
    \draw[->, blue, thick] (6, -1) tonode[midway, above] {$\scriptstyle\bar{d} / 2$}(8, -3);
    
    \draw[->, red, thick] (6, -3) to[out=45, in=135]node[midway, above] {$\scriptstyled / 2$}(8, -3);
    \draw[->, blue, thick] (6, -3) to[out=-45, in=-135]node[midway, above] {$\scriptstyled / 2$}(8, -3);
    % \draw[->, red, thick] (0, 3) to[out=30, in=150] (2, 1);
    % \node at (1, 3.5) {$d / 2$};
    % % Blue arrow from (2, 1) to (0, -1)
    % \draw[->, blue, thick] (2, 1) to[out=210, in=330] (0, -1);
    % \node at (1, 0) {$d / 2$};

    % % Additional arrows (red and blue for different connections)
    % \draw[->, red, thick] (2, 1) to[out=30, in=150] (4, 3);
    % \node at (3, 2.5) {$\overline{d}/2$};

    % \draw[->, blue, thick] (4, 3) to[out=210, in=30] (2, -1);
    % \node at (3, 1) {$\overline{d}/2$};

    % Add e labels below the columns
    \node at (1, -4) {$e_1$};
    \node at (3, -4) {$e_2$};
    \node at (5, -4) {$e_3$};
    \node at (7, -4) {$e_4$};

\end{tikzpicture}

==> figures/plots/archive/c-uiid-mi-del-rate-archive.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{chocolate2267451}{RGB}{226,74,51}
\definecolor{dimgray85}{RGB}{85,85,85}
\definecolor{gainsboro229}{RGB}{229,229,229}
\definecolor{darkblue}{RGB}{0, 0, 139}
\definecolor{darkred}{RGB}{139, 0, 0}
\definecolor{darkgreen}{RGB}{0, 100, 0}
\definecolor{darkgray}{RGB}{169, 169, 169}
\definecolor{midnightblue}{RGB}{25, 25, 112}
\definecolor{darkslategray}{RGB}{47, 79, 79}
\definecolor{darkolivegreen}{RGB}{85, 107, 47}
\definecolor{darkviolet}{RGB}{148, 0, 211}
\definecolor{darkorange}{RGB}{255, 140, 0}
\definecolor{darkmagenta}{RGB}{139, 0, 139}
\begin{axis}[
% axis background/.style={fill=gainsboro229},
width=3.675in,
height=3.45in,
%axis line style={white},
% log basis y={10},
%tick align=outside,
%tick pos=left,
x grid style={gainsboro229},
xlabel=\textcolor{dimgray85}{\(\displaystyle \delta\)},
xmajorgrids,
xmin=0.0, xmax=0.2,
% xtick style={color=dimgray85},
xticklabel style={color=dimgray85, /pgf/number format/.cd, fixed, fixed zerofill, precision=2},
y grid style={gainsboro229},
ylabel=\textcolor{dimgray85}{Information rate},
ymajorgrids,
ymin=0.0, ymax=1.0,
% ymode=log,
ymajorticks=true,
% ytick style={color=dimgray85},
legend cell align={left},
legend style={at={(1.05,0.5)}, anchor=west, nodes={scale=0.85, transform shape}},
]
\addplot [dashed, darkblue, mark=*, mark size=1, mark options={solid}]
table {%	
0.025 0.8674793510004056
0.05  0.7422946646684018
0.075 0.6565342020999515
0.1	  0.5707393786359048
0.125 0.48415078899393116
0.15  0.4299166349887853
0.175 0.37314742432660464
0.2   0.32373463993524815
};
\addlegendentry{NPD $N=64, \sF=32, \sK=32$};
\addplot [dashed, darkred, mark=*, mark size=1, mark options={solid}]
table {%	
0.025 0.8482707135532588
0.05  0.7277027210877172
0.075 0.6244447340056333
0.1   0.537145428798027
0.125 0.4538502775305495
0.15  0.38872596864707065
0.175 0.3135104959949947
0.2   0.26412776497880563
};
\addlegendentry{NPD $N=128,\sF=32, \sK=32$};
\addplot [dashed, darkgray, mark=*, mark size=1, mark options={solid}]
table {%	
0.025 0.8485837169667682
0.05  0.72410689548662
0.075 0.6229088891498893
0.1   0.5300067905511466
0.125 0.45256581013449065
0.15  0.386584642014094
0.175 0.325026825554516
0.2   0.27834998207788914
};
\addlegendentry{NPD $N=128,\sF=64, \sK=64$};
\addplot [dashed, darkgreen, mark=*, mark size=1, mark options={solid}]
table {%	
0.025 0.8317022872587274
0.05  0.6882732735087793
0.075 0.5493448732569536
0.1   0.41873847308552253
0.125 0.3404886079251473
0.15  0.2810363543201798
0.175 0.23450073640934466
0.2	  0.1996067217803935 
};
\addlegendentry{NPD $N=256,\sF=32, \sK=32$};
\addplot [dashed, darkviolet, mark=*, mark size=1, mark options={solid}]
table {%	
0.025	0.8343183757285532
0.05	0.7049736842204056
0.075	0.5913383750490157
0.1	    0.5098557968252295
0.125	0.4313501438182743
0.15	0.3471172251611588
0.175	0.2861556021078345
0.2	    0.23129587624068723
};
\addlegendentry{NPD $N=256,\sF=64, \sK=64$};
\addplot [solid, black, mark=triangle, mark size=2, mark options={solid}]
table {%
0.0   1.0  
0.05  0.747173  
0.10  0.589036  
0.15  0.468624  
0.20  0.372702  
0.25  0.294883  
0.30  0.231322  
0.35  0.179401  
0.40  0.137187  
0.45  0.10316   
0.50  0.076071  
0.55  0.054854  
0.60  0.038574  
0.65  0.026395  
0.70  0.01756   
0.75  0.011376  
0.80  0.007211  
0.85  0.004498  
0.90  0.002775  
0.95  0.001728  
1.0   0.00  
};
\addlegendentry{$\sC_\mathsf{uiid}$ UB \cite{pernice2024mutual}};

\addplot [solid, black, mark=triangle, mark size=2, mark options={solid, rotate=180}]
table {%
0.0	    1.0
0.025	0.8313390685033297
0.05	0.7136030428840439
0.075	0.615688455873503
0.1	    0.5310044064107188
0.125	0.4564355568004036
0.15	0.3901596952835995
0.175	0.3309841649434424
0.2	    0.2780719051126377
0.225	0.23080717098698622
0.25	0.18872187554086717
0.275	0.15145182170538418
0.3	    0.1187091007693073
0.325	0.0902638774688338
0.35	0.06593194462450891
0.375	0.04556599707503506
0.4	    0.02904940554533142
0.425	0.01629173737681433
0.45	0.007225546012191719
0.475	0.0018041209571899586
0.5	    0.0
};
\addlegendentry{$\sC_\mathsf{uiid}$  LB $1-h(\delta)$};

\end{axis}

\end{tikzpicture}


==> figures/plots/archive/c-uiid-mi-del-rate-att-emb.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{chocolate2267451}{RGB}{226,74,51}
\definecolor{dimgray85}{RGB}{85,85,85}
\definecolor{gainsboro229}{RGB}{229,229,229}
\definecolor{darkblue}{RGB}{0, 0, 139}
\definecolor{darkred}{RGB}{139, 0, 0}
\definecolor{darkgreen}{RGB}{0, 100, 0}
\definecolor{darkgray}{RGB}{169, 169, 169}
\definecolor{midnightblue}{RGB}{25, 25, 112}
\definecolor{darkslategray}{RGB}{47, 79, 79}
\definecolor{darkolivegreen}{RGB}{85, 107, 47}
\definecolor{darkviolet}{RGB}{148, 0, 211}
\definecolor{darkorange}{RGB}{255, 140, 0}
\definecolor{darkmagenta}{RGB}{139, 0, 139}
\begin{axis}[
% axis background/.style={fill=gainsboro229},
width=3.675in,
height=3.45in,
%axis line style={white},
% log basis y={10},
%tick align=outside,
%tick pos=left,
x grid style={gainsboro229},
xlabel=\textcolor{dimgray85}{\(\displaystyle \delta\)},
xmajorgrids,
xmin=0.02, xmax=0.11,
% xtick style={color=dimgray85},
xticklabel style={color=dimgray85, /pgf/number format/.cd, fixed, fixed zerofill, precision=2},
y grid style={gainsboro229},
ylabel=\textcolor{dimgray85}{Information rate},
ymajorgrids,
ymin=0.45, ymax=0.9,
% ymode=log,
ymajorticks=true,
% ytick style={color=dimgray85},
legend cell align={left},
legend style={at={(1.05,0.5)}, anchor=west, nodes={scale=0.85, transform shape}},
]
\addplot [only marks, darkviolet, mark=*, mark size=1, mark options={solid}]
table {%	
0.025	0.8658
0.1	    0.5679
};
\addlegendentry{NPD $N=64, e=64, h=512$};
\addplot [only marks, darkviolet, mark=square, mark size=1, mark options={solid}]
table {%	
0.025	0.8696
0.1	    0.590
};
\addlegendentry{NPD $N=64, e=256, h=512$};



\addplot [only marks, darkblue, mark=*, mark size=1, mark options={solid}]
table {%	
0.025	0.8214
0.1	    0.5369
};
\addlegendentry{NPD $N=128, e=64, h=512$};
\addplot [only marks, darkblue, mark=square, mark size=1, mark options={solid}]
table {%	
0.025	0.8541
0.1	    0.5561
};
\addlegendentry{NPD $N=128, e=256, h=512$};



\addplot [only marks, darkred, mark=*, mark size=1, mark options={solid}]
table {%	
0.025	0.8382
0.1	    0.4966
};
\addlegendentry{NPD $N=256, e=64, h=512$};
\addplot [only marks, darkred, mark=square, mark size=1, mark options={solid}]
table {%	
0.025	0.8421
0.1	    0.5254
};
\addlegendentry{NPD $N=256, e=256, h=512$};



\addplot [only marks, darkgreen, mark=*, mark size=1, mark options={solid}]
table {%	
0.025	0.8114
0.1	    0.4621
};
\addlegendentry{NPD $N=512, e=64, h=512$};
\addplot [only marks, darkgreen, mark=square, mark size=1, mark options={solid}]
table {%	
0.025	0.8107
0.1	    0.5074
};
\addlegendentry{NPD $N=512, e=256, h=512$};
\addplot [only marks, darkgreen, mark=o, mark size=1, mark options={solid}]
table {%	
0.025	0.8252
0.1	    0.5244
};
\addlegendentry{NPD $N=512, e=256, h=1024$};



\addplot [only marks, darkorange, mark=*, mark size=1, mark options={solid}]
table {%	
0.025	0.7449
0.1	    0.4813
};
\addlegendentry{NPD $N=1024, e=256, h=1024$};
\addplot [only marks, darkorange, mark=square, mark size=1, mark options={solid}]
table {%	
0.025	0.7994
0.1	    0.4812
};
\addlegendentry{NPD $N=1024, e=512, h=2048$};
\addplot [only marks, darkorange, mark=o, mark size=1, mark options={solid}]
table {%	
0.1	    0.5244
};
\addlegendentry{NPD $N=1024, e=768, h=2048$};

\addplot [solid, black, mark=triangle, mark size=0.1, mark options={solid}]
table {%
0.0   1.0  
0.05  0.747173  
0.10  0.589036  
0.15  0.468624  
0.20  0.372702  
0.25  0.294883  
0.30  0.231322  
0.35  0.179401  
0.40  0.137187  
0.45  0.10316   
0.50  0.076071  
0.55  0.054854  
0.60  0.038574  
0.65  0.026395  
0.70  0.01756   
0.75  0.011376  
0.80  0.007211  
0.85  0.004498  
0.90  0.002775  
0.95  0.001728  
1.0   0.00  
};
\addlegendentry{$\sC_\mathsf{uiid}$ UB \cite{pernice2024mutual}};

\addplot [solid, black, mark=triangle, mark size=0.1, mark options={solid, rotate=180}]
table {%
0.0	    1.0
0.025	0.8313390685033297
0.05	0.7136030428840439
0.075	0.615688455873503
0.1	    0.5310044064107188
0.125	0.4564355568004036
0.15	0.3901596952835995
0.175	0.3309841649434424
0.2	    0.2780719051126377
0.225	0.23080717098698622
0.25	0.18872187554086717
0.275	0.15145182170538418
0.3	    0.1187091007693073
0.325	0.0902638774688338
0.35	0.06593194462450891
0.375	0.04556599707503506
0.4	    0.02904940554533142
0.425	0.01629173737681433
0.45	0.007225546012191719
0.475	0.0018041209571899586
0.5	    0.0
};
\addlegendentry{$\sC_\mathsf{uiid}$  LB $1-h(\delta)$};

\end{axis}

\end{tikzpicture}


==> figures/plots/archive/c-uiid-mi-del-rate-cnn-emb.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{chocolate2267451}{RGB}{226,74,51}
\definecolor{dimgray85}{RGB}{85,85,85}
\definecolor{gainsboro229}{RGB}{229,229,229}
\definecolor{darkblue}{RGB}{0, 0, 139}
\definecolor{darkred}{RGB}{139, 0, 0}
\definecolor{darkgreen}{RGB}{0, 100, 0}
\definecolor{darkgray}{RGB}{169, 169, 169}
\definecolor{midnightblue}{RGB}{25, 25, 112}
\definecolor{darkslategray}{RGB}{47, 79, 79}
\definecolor{darkolivegreen}{RGB}{85, 107, 47}
\definecolor{darkviolet}{RGB}{148, 0, 211}
\definecolor{darkorange}{RGB}{255, 140, 0}
\definecolor{darkmagenta}{RGB}{139, 0, 139}
\begin{axis}[
% axis background/.style={fill=gainsboro229},
width=3.675in,
height=3.45in,
%axis line style={white},
% log basis y={10},
%tick align=outside,
%tick pos=left,
x grid style={gainsboro229},
xlabel=\textcolor{dimgray85}{\(\displaystyle \delta\)},
xmajorgrids,
xmin=0.02, xmax=0.11,
% xtick style={color=dimgray85},
xticklabel style={color=dimgray85, /pgf/number format/.cd, fixed, fixed zerofill, precision=2},
y grid style={gainsboro229},
ylabel=\textcolor{dimgray85}{Information rate},
ymajorgrids,
ymin=0.45, ymax=0.9,
% ymode=log,
ymajorticks=true,
% ytick style={color=dimgray85},
legend cell align={left},
legend style={at={(1.05,0.5)}, anchor=west, nodes={scale=0.85, transform shape}},
]
\addplot [only marks, darkviolet, mark=*, mark size=1, mark options={solid}]
table {%	
0.025	0.873
0.1	    0.590
};
\addlegendentry{NPD $N=64, e=256, h=1024$};



\addplot [only marks, darkblue, mark=*, mark size=1, mark options={solid}]
table {%	
0.025	0.8539
0.1	    0.5487
};
\addlegendentry{NPD $N=128, e=256, h=1024$};




\addplot [only marks, darkred, mark=*, mark size=1, mark options={solid}]
table {%	
0.025	0.8396
% 0.1	    0.4966
};
\addlegendentry{NPD $N=256, e=256, h=1024$};




\addplot [only marks, darkgreen, mark=*, mark size=1, mark options={solid}]
table {%	
0.025	0.827
% 0.1	    0.4621
};
\addlegendentry{NPD $N=512, e=512, h=2048$};




\addplot [only marks, darkorange, mark=*, mark size=1, mark options={solid}]
table {%	
0.025	0.79
% 0.1	    0.4813
};
\addlegendentry{NPD $N=1024, e=1024, h=2048$};


\addplot [solid, black, mark=triangle, mark size=0.1, mark options={solid}]
table {%
0.0   1.0  
0.05  0.747173  
0.10  0.589036  
0.15  0.468624  
0.20  0.372702  
0.25  0.294883  
0.30  0.231322  
0.35  0.179401  
0.40  0.137187  
0.45  0.10316   
0.50  0.076071  
0.55  0.054854  
0.60  0.038574  
0.65  0.026395  
0.70  0.01756   
0.75  0.011376  
0.80  0.007211  
0.85  0.004498  
0.90  0.002775  
0.95  0.001728  
1.0   0.00  
};
\addlegendentry{$\sC_\mathsf{uiid}$ UB \cite{pernice2024mutual}};

\addplot [solid, black, mark=triangle, mark size=0.1, mark options={solid, rotate=180}]
table {%
0.0	    1.0
0.025	0.8313390685033297
0.05	0.7136030428840439
0.075	0.615688455873503
0.1	    0.5310044064107188
0.125	0.4564355568004036
0.15	0.3901596952835995
0.175	0.3309841649434424
0.2	    0.2780719051126377
0.225	0.23080717098698622
0.25	0.18872187554086717
0.275	0.15145182170538418
0.3	    0.1187091007693073
0.325	0.0902638774688338
0.35	0.06593194462450891
0.375	0.04556599707503506
0.4	    0.02904940554533142
0.425	0.01629173737681433
0.45	0.007225546012191719
0.475	0.0018041209571899586
0.5	    0.0
};
\addlegendentry{$\sC_\mathsf{uiid}$  LB $1-h(\delta)$};

\end{axis}

\end{tikzpicture}


==> figures/plots/archive/nanopore_compare_scatter.tex <==
\begin{tikzpicture}
    \definecolor{chocolate2267451}{RGB}{226,74,51}
    \definecolor{dimgray85}{RGB}{85,85,85}
    \definecolor{gainsboro229}{RGB}{229,229,229}
    \definecolor{darkblue}{RGB}{0, 0, 139}
    \definecolor{darkred}{RGB}{139, 0, 0}
    \definecolor{darkgreen}{RGB}{0, 100, 0}
    \definecolor{darkgray}{RGB}{169, 169, 169}
    \definecolor{midnightblue}{RGB}{25, 25, 112}
    \definecolor{darkslategray}{RGB}{47, 79, 79}
    \definecolor{darkolivegreen}{RGB}{85, 107, 47}
    \definecolor{darkviolet}{RGB}{148, 0, 211}
    \definecolor{darkorange}{RGB}{255, 140, 0}
    \definecolor{darkmagenta}{RGB}{139, 0, 139}
    \begin{axis}[
        width=3.54in,
        height=2.76in,
        ylabel=\textcolor{dimgray85}{FER},
        xlabel=\textcolor{dimgray85}{Number of parameters},
        ymin=0,
        xtick=data,
        xmode=log,
        % xticklabel style={rotate=45, anchor=east},
        % xticklabels={NPD, DNAformer, Iterative, BMA Lookahead, BMA Trellis, Divider BMA, VS},
        every axis/.append style={
            label style={text=dimgray85},
            tick label style={text=dimgray85}},
        ]
        \addplot[
            only marks,
            mark=*,
            color=darkgreen,
            ] coordinates {
                (3294594, 0.1494)
                (100000000, 0.1458)
                (100, 0.1672)
                (100, 0.3144)
                (100, 0.8477)
                (100, 0.9136)
                (100, 0.9435)
            };
    \end{axis}
\end{tikzpicture}

==> figures/plots/tmp/npd-ids-scl-fer.tex <==
    \begin{tikzpicture}
\definecolor{chocolate2267451}{RGB}{226,74,51}
\definecolor{dimgray85}{RGB}{85,85,85}
\definecolor{gainsboro229}{RGB}{229,229,229}
\definecolor{darkblue}{RGB}{0, 0, 139}
\definecolor{darkred}{RGB}{139, 0, 0}
\definecolor{darkgreen}{RGB}{0, 100, 0}
\definecolor{darkgray}{RGB}{169, 169, 169}
\definecolor{midnightblue}{RGB}{25, 25, 112}
\definecolor{darkslategray}{RGB}{47, 79, 79}
\definecolor{darkolivegreen}{RGB}{85, 107, 47}
\definecolor{darkviolet}{RGB}{148, 0, 211}
\definecolor{darkorange}{RGB}{255, 140, 0}
\definecolor{darkmagenta}{RGB}{139, 0, 139}
        \begin{axis}[
width=2.94in,
height=2.76in,
	xlabel={List Size $L$},
	title={$R=0.5$},
	ylabel={Frame Error Rate},
	ymode=log,
	log basis y=10,
	ytick={1e-2, 2e-2, 5e-2, 1e-1},
	yticklabels={0.01, 0.02, 0.05, 0.1},
	% ytick={0.1, 0.01, 0.001, 0.0001}, % Define the ticks explicitly
	% yticklabels={$10^{-1}$, $10^{-2}$, $10^{-3}$, $10^{-4}$}, 
	ymin=0.005, ymax=0.1,
	xtick={0, 1, 2, 3},
	xticklabels={SC,SCL2,SCL4,SCL8},
	% symbolic x coords={SC,SCL2,SCL4,SCL8},
	% ytick=data,
	grid=both,
	legend pos=north east,
	legend style={font=\small}
	]
	
	\addplot[
	color=green,
	mark=o,
	thick
	] 
	table {
		0 0.049660
		1 0.032368
		2 0.029670
		3 0.027372 
	};
	% coordinates {
		% (0, 4.802e-02) (1, 3.743e-02) (2, 3.650e-02) (3, 3.588e-02)
		% };
	\addlegendentry{$N=32$}
	
	\addplot[
	color=blue,
	mark=square*,
	thick
	] table {
		0 0.046354
		1 2.897e-02
		2 2.557e-02
		3 2.325e-02
	};
	\addlegendentry{$N=64$}
	
	\addplot[
	color=red,
	mark=triangle*,
	thick
	] table {
		0 0.032967
		1 0.015986
		2 0.010589
		3 0.00959
	};
	\addlegendentry{$N=128$}
	
	\addplot[
	color=purple,
	mark=diamond*,
	thick
	] table {
		0 0.02327
		1 0.012788
		2 0.009888
		3 0.009210
	};
	\addlegendentry{$N=256$}
	\addplot[
	color=orange,
	mark=star,
	thick
	] table {
		0 1.768e-02
		1 8.463e-03
		2 7.293e-03
		3 7.121e-03
	};
	\addlegendentry{$N=512$}
\end{axis}
\end{tikzpicture}

==> figures/plots/tmp/scl-deletion-d-0.1-n-256.tex <==
\begin{tikzpicture}
\definecolor{chocolate2267451}{RGB}{226,74,51}
\definecolor{dimgray85}{RGB}{85,85,85}
\definecolor{gainsboro229}{RGB}{229,229,229}
\definecolor{darkblue}{RGB}{0, 0, 139}
\definecolor{darkred}{RGB}{139, 0, 0}
\definecolor{darkgreen}{RGB}{0, 100, 0}
\definecolor{darkgray}{RGB}{169, 169, 169}
\definecolor{midnightblue}{RGB}{25, 25, 112}
\definecolor{darkslategray}{RGB}{47, 79, 79}
\definecolor{darkolivegreen}{RGB}{85, 107, 47}
\definecolor{darkviolet}{RGB}{148, 0, 211}
\definecolor{darkorange}{RGB}{255, 140, 0}
\definecolor{darkmagenta}{RGB}{139, 0, 139}
\begin{axis}[
    width=10cm, height=8cm,
    xlabel={\textcolor{dimgray85}{\(\displaystyle R\)}},
    ylabel={\textcolor{dimgray85}{BER}},
    ymode=log,
    log basis y=10,
    colorbar,
    colormap/viridis,
    legend style={at={(1.05,1)}, anchor=north west},
    % scatter/classes={
    %     1={mark=*,darkblue},
    %     2={mark=square*,darkred},
    %     4={mark=triangle*,green},
    %     8={mark=diamond*,purple}
    % },
    colorbar style={
      title={\textcolor{dimgray85}{\(\displaystyle L\)}},
      ymode=log,
      log basis y=2,
      % ytick={0, 1, 2, 3, 4},
      % yticklabels={$1$, $2$, $4$, $8$, $16$},
    },
    point meta min=1,    % Minimum value for the color bar
    point meta max=5,   
    scatter src=explicit,
    % scatter src=explicit symbolic,
]

% Scatter plot for all points
\addplot[
    scatter,only marks,
    point meta=explicit,
] table  [
    x={Code-Rate},
    y={BER},
    meta={L},
    col sep=comma,
] {./figures/ber_fer_del-0.1_n-256-e256-h-2048-l2.csv};


\end{axis}
\end{tikzpicture}




% \begin{tikzpicture}
% \definecolor{darkblue}{rgb}{0,0,0.55}
% \definecolor{darkgreen}{rgb}{0,0.39,0}
% \definecolor{maroon}{rgb}{0.5,0,0}
% \definecolor{plum}{rgb}{0.56,0.27,0.52}
% \definecolor{darkorange}{rgb}{0.8,0.33,0} 
% \definecolor{dimgray85}{RGB}{85,85,85}
% \definecolor{gainsboro229}{RGB}{229,229,229}



% % First plot
% \begin{axis}[
%     name=plot1,
%     title={Optimized Input Distribution},
%     xlabel={\textcolor{dimgray85}{$\displaystyle \log_2(N)$}},
%     ylabel={\textcolor{dimgray85}{BER}},
%     ymode=log,
%     ymin=5e-4, ymax=0.3,
%     xmajorgrids,
%     ymajorgrids,
%     % colorbar,
%     colormap/viridis,
%     % colorbar style={
%     %   title={$L$},
%     %   ytick={0, 2, 4, 6, 8},
%     %   yticklabels={$1$, $4$, $16$, $64$, $256$},
%     % },
%   ]
%     \addplot [scatter,
%       only marks,
%       scatter src=explicit,
%     ]
%     table[meta expr=log10(\thisrow{meta})/log10(2)]{
% n	ber	meta
% 3	0.033479927	1
% 3	0.017758224	2
% 3	0.017571576463974736	4
% 3	0.016834983450748266	8
% 3	0.016355031	16
% 3	0.017031630454999353	32
% 3	0.017064801210585026	64
% 3	0.017537897997412427	128
% 3	0.016841579483545522	256
% 4	0.032335499369281935	1
% 4	0.008772281	2
% 4	0.005345661	4
% 4	0.005450608	8
% 4	0.004907546	16
% 4	0.005197401	32
% 4	0.005125771	64
% 4	0.005265701	128
% 4	0.005312344	256
% 5	0.06629935	1
% 5	0.025696318692144664	2
% 5	0.017428785806846644	4
% 5	0.016709145630734494	8
% 5	0.016692487289761377	16
% 5	0.016605031018790933	32
% 5	0.016449275560777583	64
% 5	0.016458437647791518	128
% 5	0.016085291	256
% 6	0.061116642	1
% 6	0.020843178262298312	2
% 6	0.010864567562066454	4
% 6	0.008676062	8
% 6	0.008474563	16
% 6	0.008370215	32
% 6	0.008215492	64
% 6	0.008290255	128
% 6	0.008245077	256
% 7	0.12754152651340037	1
% 7	0.041108466400925456	2
% 7	0.012919422964389058	4
% 7	0.005710674	8
% 7	0.004218675	16
% 7	0.003954101	32
% 7	0.003712066	64
% 7	0.003839257	128
% 7	0.003671694	256
% 8	0.13120097094537994	1
% 8	0.042359018	2
% 8	0.012508353983610124	4
% 8	0.005933798	8
% 8	0.004140381	16
% 8	0.003405944	32
% 8	0.003370374	64
% 8	0.003267386	128
% 8	0.00329012	256
% 9	0.1859047440439323	1
% 9	0.072498114	2
% 9	0.028696583345581752	4
% 9	0.011699738529972036	8
% 9	0.005831986	16
% 9	0.003715201	32
% 9	0.002892965	64
% 9	0.002483954	128
% 9	0.002379154	256
% 10	0.23510296203503464	1
% 10	0.090695972	2
% 10	0.030658045058436077	4
% 10	0.011330618318891724	8
% 10	0.0046336	16
% 10	0.002252786	32
% 10	0.00128437	64
% 10	0.000807591	128
% 10	0.000670569	256
% };

% \addplot[dimgray85, line width=0.1pt] coordinates {(3,0.033479927) (4,0.032335499369281935) (5,0.06629935) (6,0.061116642) (7,0.12754152651340037) (8,0.13120097094537994) (9,0.1859047440439323) (10,0.23510296203503464)};
% \addplot[dimgray85, line width=0.1pt] coordinates {(3,0.017758224) (4,0.008772281) (5,0.025696318692144664) (6,0.020843178262298312) (7,0.041108466400925456) (8,0.042359018) (9,0.072498114) (10,0.090695972)};
% \addplot[dimgray85, line width=0.1pt] coordinates {(3,0.017571576463974736) (4,0.005345661) (5,0.017428785806846644) (6,0.010864567562066454) (7,0.012919422964389058) (8,0.012508353983610124) (9,0.028696583345581752) (10,0.030658045058436077)};
% \addplot[dimgray85, line width=0.1pt] coordinates {(3,0.016834983450748266) (4,0.005450608) (5,0.016709145630734494) (6,0.008676062) (7,0.005710674) (8,0.005933798) (9,0.011699738529972036) (10,0.011330618318891724)};
% \addplot[dimgray85, line width=0.1pt] coordinates {(3,0.016355031) (4,0.004907546) (5,0.016692487289761377) (6,0.008474563) (7,0.004218675) (8,0.004140381) (9,0.005831986) (10,0.0046336)};
% \addplot[dimgray85, line width=0.1pt] coordinates {(3,0.017031630454999353) (4,0.005197401) (5,0.016605031018790933) (6,0.008370215) (7,0.003954101) (8,0.003405944) (9,0.003715201) (10,0.002252786)};
% \addplot[dimgray85, line width=0.1pt] coordinates {(3,0.017064801210585026) (4,0.005125771) (5,0.016449275560777583) (6,0.008215492) (7,0.003712066) (8,0.003370374) (9,0.002892965) (10,0.00128437)};
% \addplot[dimgray85, line width=0.1pt] coordinates {(3,0.017537897997412427) (4,0.005265701) (5,0.016458437647791518) (6,0.008290255) (7,0.003839257) (8,0.003267386) (9,0.002483954) (10,0.000807591)};
% \addplot[dimgray85, line width=0.1pt] coordinates {(3,0.016841579483545522) (4,0.005312344) (5,0.016085291) (6,0.008245077) (7,0.003671694) (8,0.00329012) (9,0.002379154) (10,0.000670569)};

% \end{axis}


% \end{tikzpicture}
